The symplectic properties of the PGL(n,C)-gluing equations

In a previous article we studied PGL(n,C)-representations of a 3-manifold via a generalization of Thurston's gluing equations. Neumann has proved some symplectic properties of Thurston's gluing equations that play an important role in recent developments of exact and perturbative Chern-Simons theory. In this paper, we prove the symplectic properties of the PGL(n,C)-gluing equations for all ideal triangulations of compact oriented 3-manifolds.

==> BetaStarFace.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(341.45306,303.14847)
 \put(0,0){\includegraphics{BetaStarFace_included}}

\definecolor{inkcol1}{rgb}{0.0,0.0,0.0}
   \put(185.536283,161.993586){\rotatebox{360.0}{\makebox(0,0)[tl]{\strut{}{
    \begin{minipage}[h]{127.655896pt}
\textcolor{inkcol1}{\LARGE{$t$}}\\
\end{minipage}}}}}%

 \end{picture}
\endgroup


==> EdgePath.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(402.54099,187.929)
 \put(0,0){\includegraphics{EdgePath_included}}
 \end{picture}
\endgroup


==> SchematicEdgeGluing.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(174.74625,187.87822)
 \put(0,0){\includegraphics{SchematicEdgeGluing_included}}
 \end{picture}
\endgroup


==> SchematicFaceGluing.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(236.35715,159.57143)
 \put(0,0){\includegraphics{SchematicFaceGluing_included}}
 \end{picture}
\endgroup


==> mathdots.tex <==
%%
%% This is file `mathdots.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% mathdots.dtx  (with options: `tex')
%% 
%% -------------------------------------------------------------------
%% 
%% Copyright 2001--2006, Daniel H. Luecking
%% 
%% Mathdots may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License, either version 1.3 of this license or (at
%% your option) any later version. The latest version of this license is in
%%    <http://www.latex-project.org/lppl.txt>
%% and version 1.3 or later is part of all distributions of LaTeX version
%% 2003/12/01 or later.
%% 
%% Mathdots has maintenance status "author-maintained". The Current
%% Maintainer is Daniel H. Luecking. The Base Interpreters associated with
%% mathdots are plain TeX and LaTeX
%% 
\def\mathdotsfiledate{2006/03/16}%
\def\mathdotsfileversion{0.8}%
\expandafter
\ifx\csname MathDots\mathdotsfileversion\endcsname\relax
\else
  \immediate\write16{Mathdots already loaded.}\expandafter\endinput
\fi
\immediate\write16{Package mathdots, \mathdotsfiledate\space version
  \mathdotsfileversion.}%
\expandafter\edef\csname MathDots\mathdotsfileversion\endcsname{%
    \catcode`\noexpand\@=\the\catcode`@}%
\catcode`\@=11
\def\@nameuse#1{\csname#1\endcsname}%
\def\MD@us#1{\@nameuse{#1style}}%
\def\MD@uf#1{\@nameuse{#1font}0}%
\def\MD@t{text}\def\MD@s{script}\def\MD@ss{scriptscript}%
\newdimen\MD@unit \MD@unit\p@
\def\MD@changestyle#1{\relax\MD@unit0.1\fontdimen6\MD@uf{#1}%
  \everymath\expandafter{\the\everymath\MD@us{#1}}}%
\def\MD@dot{$\m@th\ldotp$}%
\def\MD@palette#1{\mathchoice{#1\MD@t}{#1\MD@t}{#1\MD@s}{#1\MD@ss}}%
\def\MD@ddots#1{{\MD@changestyle{#1}%
  \mkern1mu\raise7\MD@unit\vbox{\kern7\MD@unit\hbox{\MD@dot}}%
  \mkern2mu\raise4\MD@unit\hbox{\MD@dot}%
  \mkern2mu\raise \MD@unit\hbox{\MD@dot}\mkern1mu}}%
\def\MD@vdots#1{\vbox{\MD@changestyle{#1}%
  \baselineskip4\MD@unit\lineskiplimit\z@
  \kern6\MD@unit\hbox{\MD@dot}\hbox{\MD@dot}\hbox{\MD@dot}}}%
\def\MD@iddots#1{{\MD@changestyle{#1}%
  \mkern1mu\raise \MD@unit\hbox{\MD@dot}%
  \mkern2mu\raise4\MD@unit\hbox{\MD@dot}%
  \mkern2mu\raise7\MD@unit\vbox{\kern7\MD@unit\hbox{\MD@dot}}}}%
\def\fixedvdots{%
  \vbox{\baselineskip4\p@ \lineskiplimit\z@
  \kern6\p@\hbox{.}\hbox{.}\hbox{.}}}%
\def\fixedddots{%
  \mathinner{\mkern1mu
  \raise7\p@\vbox{\kern7\p@\hbox{.}}\mkern2mu
  \raise4\p@\hbox{.}\mkern2mu
  \raise\p@\hbox{.}\mkern1mu}}%
\def\fixediddots{%
  \mathinner{\mkern1mu
  \raise\p@\hbox{.}\mkern2mu
  \raise4\p@\hbox{.}\mkern2mu
  \raise7\p@\vbox{\kern7\p@\hbox{.}}\mkern1mu}}%
\let\originalddots=\ddots
\let\originalvdots=\vdots
\let\originaliddots=\iddots
\def\ddots{%
  \mathinner{\MD@palette\MD@ddots}}%
\def\iddots{%
  \mathinner{\MD@palette\MD@iddots}}%
\def\vdots{%
  \mathinner{\MD@palette\MD@vdots}}%
\wlog{Mathdots Info: Redefining \string\ddots.}%
\wlog{Mathdots Info: Redefining \string\vdots.}%
\newbox\MD@dotsbox
\newmuskip\MD@prekern
\newmuskip\MD@postkern
\newmuskip\MD@dotkern
\MD@prekern 0mu
\MD@postkern -1mu
\MD@dotkern -1.3mu
\def\MD@dotsaccent#1{\mathpalette{\MD@@dotsaccent{#1}}}%
\def\MD@@dotsaccent#1#2#3{%
  {\setbox\MD@dotsbox\hbox{$#2\mkern\MD@prekern#1\mkern\MD@postkern$}%
   \mathop{#3\kern\z@}\limits^{%
   \text{\vbox to-1.4\ex@{\kern-1.8\ex@\copy\MD@dotsbox\vss}}}}%
}%
\let\originaldddot \dddot
\let\originalddddot\ddddot
\def\amstexfmtname{AmS-TeX}%
\ifx\amstexfmtname\fmtname
  \def\MD@D{\mathchar"5F\mkern\MD@dotkern}%
  \wlog{Mathdots Info: Redefining \string\dddot.}%
  \wlog{Mathdots Info: Redefining \string\ddddot.}%
  \def\dddot {\MD@dotsaccent{\MD@D\MD@D\MD@D}}%
  \def\ddddot{\MD@dotsaccent{\MD@D\MD@D\MD@D\MD@D}}%
\fi
\csname MathDots\mathdotsfileversion\endcsname
\endinput
%%
%% End of file `mathdots.tex'.

